Autonomous Gaussian decomposition of the Galactic Ring Survey. I. Global statistics and properties of the 13CO emission data

The analysis of large molecular line surveys of the Galactic plane is essential for our understanding of the gas kinematics on Galactic scales, in particular its link with the formation and evolution of dense structures in the interstellar medium. An approximation of the emission peaks with Gaussian functions allows for an efficient and straightforward extraction of useful physical information contained in the shape and Doppler-shifted frequency of the emission lines contained in these enormous data sets. In this work we present an overview and first results of a Gaussian decomposition of the entire Galactic Ring Survey (GRS) 13CO (1-0) data that consists of about 2.3 million spectra. We performed the decomposition with the fully automated GaussPy+ algorithm and fitted about 4.6 million Gaussian components to the GRS spectra. We discuss the statistics of the fit components and relations between the fitted intensities, velocity centroids, and velocity dispersions. We find that the magnitude of the velocity dispersion values increase toward the inner Galaxy and around the Galactic midplane, which we speculate is partly due to the influence of the Galactic bar and regions with higher non-thermal motions located in the midplane, respectively. We also use our decomposition results to infer global properties of the gas emission and find that the number of fit components used per spectrum is indicative for the amount of structure along the line of sight. We find that the emission lines from regions located on the far side of the Galaxy show increased velocity dispersion values, likely due to beam averaging effects. We demonstrate how this trend has the potential to aid in characterising Galactic structure by disentangling emission that is belonging to the nearby Aquila Rift molecular cloud from emission that is more likely associated with the Perseus and Outer spiral arms.

==> symbols.tex <==
% Local symbols
\newcommand{\kb}{k_{\mathrm{B}}}
\newcommand{\msun}{M$_\text{\odot}$}
\newcommand{\rsun}{R_{\odot}}
\newcommand{\lsun}{L_{\odot}}
\newcommand{\avir}{\alpha_{\mathrm{vir}}}
\newcommand{\vecr}{\mathbf{r}}
\newcommand{\vecv}{\mathbf{v}}
\newcommand{\vecg}{\mathbf{g}}
\newcommand{\vecx}{\mathbf{x}}
\newcommand{\veck}{\mathbf{k}}
\newcommand{\vecB}{\mathbf{B}}
\newcommand{\vecf}{\mathbf{f}}
\newcommand{\nhat}{\hat{\mathbf{n}}}
\newcommand{\vecS}{\mathbf{S}}
\newcommand{\vecI}{\mathbf{I}}
\newcommand{\vecPi}{\boldsymbol{\Pi}}
\newcommand{\vecT}{\mathbf{T}}
\newcommand{\veco}{{\bm \Omega}}
\newcommand{\ehat}{\hat{\mathbf{e}}}
\newcommand{\alphab}{\alpha_{\mathrm{B}}}

% AAStex symbols
\usepackage{amssymb}

% Journals
\newcommand{\physrep}{Phys.~Rep.}
\newcommand{\aapr}{Astron.\& Astrophys.~Rev.}
\newcommand{\aap}{Astron.~\& Astrophys.}
\newcommand{\aaps}{Astron.~\& Astrophys.~Supp.}
\newcommand{\apj}{Astrophys.~J.}
\newcommand{\apjs}{Astrophys.~J.~Supp.}
\newcommand{\apjl}{Astrophys.~J.}
\newcommand{\apss}{Astrophys.~\& Space~Science}
\newcommand{\aj}{Astron.~J.}
\newcommand{\araa}{Annu.~Rev.~Astron.~Astrophys.}
\newcommand{\pasp}{Proc.~Astron.~Soc.~Pac.}
\newcommand{\mnras}{Mon.~Not.~Roy.~Astron.~Soc.}
\newcommand{\pasj}{Proc.~Astron.~Soc.~Japan}
\newcommand{\nat}{Nature}
